Featurized Density Ratio Estimation

Density ratio estimation serves as an important technique in the unsupervised machine learning toolbox. However, such ratios are difficult to estimate for complex, high-dimensional data, particularly when the densities of interest are sufficiently different. In our work, we propose to leverage an invertible generative model to map the two distributions into a common feature space prior to estimation. This featurization brings the densities closer together in latent space, sidestepping pathological scenarios where the learned density ratios in input space can be arbitrarily inaccurate. At the same time, the invertibility of our feature map guarantees that the ratios computed in feature space are equivalent to those in input space. Empirically, we demonstrate the efficacy of our approach in a variety of downstream tasks that require access to accurate density ratios such as mutual information estimation, targeted sampling in deep generative models, and classification with data augmentation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> meetings.tex <==
\section{Meeting Notes}
\texttt{https://docs.google.com/document/d/1PCjPRPXyy20iyV2egC8jSSJq1ib1QLemHCeA9qY66M8/edit}


==> sections/old.tex <==
% \begin{enumerate}
%     % \item Learning density ratio estimates using a binary classifier
%     \item Variance reduction techniques for importance sampling maybe? We could borrow the bits from Mixture Importance Sampling and Multiple Importance Sampling from the Owen chapter.
% \end{enumerate}

% \subsection{TRE (\cite{rhodes2020telescoping})}
% (Paraphrased loosely) Assume we have samples from a reference (target) dataset $x_1 \sim p(x)$ and a biased dataset $x_2 \sim q(x)$, where $x \in \mathcal{X}$. Instead of directly estimating $r(x) = \frac{p(x)}{q(x)}$, which is problematic when $p$ and $q$ are sufficiently different, TRE proposes to estimate $r(x)$ with a model $r(x; \theta)$ using a set of intermediate datsets:
% $$r(x)  = \frac{p(x)}{q(x)} \approx \prod_{i=1}^m r_i(x_i; \theta) = \frac{p(x)}{p_1(x)} \times \frac{p_1(x)}{p_2(x)} \times \cdots \times \frac{p_m(x)}{q(x)}$$
% where each $r_i(x; \theta)$ is the output of a binary classifier and $x_i$ are samples from the intermediate distributions which are obtained by interpolating between $p$ and $q$. The paper adopts a linear interpolation scheme, among others.

% The actual model is learned via multi-task learning, and is comprised of a shared body (used for learning a shared embedding scheme of each data point) and individual output heads (an individual linear layer) for each binary classification task ($p_i(x) \text{ vs. } p_{i+1}(x)$). 

% The $m$ individual logistic losses $\mathcal{L}_i$ for each head is then aggregated into a final loss:
% $$\mathcal{L_{TRE}} = \frac{1}{m}\sum_{i=1}^m \mathcal{L}_i$$

% \subsection{Toy 1-D Example}
% \subsubsection{Single source, sanity check}
% \paragraph{Dataset}
% We are working with 2 Gaussian distributions for our $p, q$, where we have 10K samples from each to verify that we can reproduce the paper's results:
% \begin{enumerate}
%     \item $x_1 \sim \mathcal{N}(0, 1e^{-6}) = p$
%     \item $x_2 \sim \mathcal{N}(0, 1) = q$
% \end{enumerate}

% \begin{figure*}[!ht]
% \centering
% \subfigure[Waymarks (Interpolations)]{\includegraphics[width=.9\linewidth]
% {figures/prelim_exp/sanity_bridge.png}}
% \subfigure[True Density Ratio]{\includegraphics[width=.4\linewidth]
% {figures/prelim_exp/sanity1.png}}
% \subfigure[Loss]{\includegraphics[width=.57\linewidth]
% {figures/prelim_exp/sanity_loss.png}}
% % \caption{test}
% % \label{fig:90_10_results}
% \end{figure*}

% \subsubsection{Multi-source Baseline}
% \paragraph{Dataset}
% We are working with 3 Gaussian distributions for our $p, q, r$, where we have 10K samples from each:
% \begin{enumerate}
%     \item $x_1 \sim \mathcal{N}(0, 1e^{-6}) = p$
%     \item $x_2 \sim \mathcal{N}(0, 1e^{-3}) = r$
%     \item $x_3 \sim \mathcal{N}(0, 1) = q$
% \end{enumerate}
% \pagebreak

% \subsection{Different classifiers}
% \begin{figure*}[ht]
%     \centering
%     \subfigure[Learned ratios]{\includegraphics[width=.47\linewidth]{figures/prelim_exp/shared_pq.png}}
%     \subfigure[True ratios]{\includegraphics[width=.47\linewidth]{figures/prelim_exp/shared_true_pq.png}}
%     \caption{Learned and true density ratio estimates for P vs. Q}
% \end{figure*}

% \subsection{MTL}
% \begin{figure*}[!ht]
% \centering
% \subfigure[Learned ratios]{\includegraphics[width=.47\linewidth]
% {figures/prelim_exp/mtl_pq.png}}
% \subfigure[True ratios]{\includegraphics[width=.47\linewidth]
% {figures/prelim_exp/mtl_true_pq.png}}
% \caption{Learned and true density ratio estimates for P vs. Q}
% \end{figure*}

% \begin{figure*}[!ht]
% \centering
% % \subfigure[Learned ratios]{\includegraphics[width=.47\linewidth]
% % {figures/prelim_exp/mtl_pr.png}}
% \subfigure[True ratios]{\includegraphics[width=.47\linewidth]
% {figures/prelim_exp/mtl_true_pr.png}}
% \caption{Learned and true density ratio estimates for P vs. R \kristy{TODO: figure out what's up here for P vs. R!!}}
% \end{figure*}

% \subsubsection{Multi-source Consistency}
% TODO

% \subsection{CelebA}
% \paragraph{Dataset} We are in the multi-attribute setting, where the 3 datasets are:
% \begin{enumerate}
%     \item 90-10 split (female, male)
%     \item 30-70 split (black hair, other colored hair)
%     \item unbiased across all 4 categories
% \end{enumerate}

% \paragraph{Different classifiers}

% \paragraph{MTL}

% \subsection{Real Datasets: TODO}
% \begin{enumerate}
%     \item Tiny-ImageNet (?)
%     \item Husky vs Wolf dataset (?)
%     \item \kristy{Brainstorm some possible ideas for similar distributions, but not exactly overlapping support}
% \end{enumerate}

% OLD
% The step-1 extension is to make TRE amenable to multiple data sources. \kristy{TODO: we'll need to do more}

% Suppose we have 1 target data source $p$ and 2 biased data sources $\{q, r\}$. We can straightforwardly train 2 classifiers to distinguish between $p/q$ and $p/r$, while taking the telescoping trick of TRE into account for each loss component:
% $$\mathcal{L}_\text{Multi-TRE} = \frac{1}{2}\left(\mathcal{L}_\text{TRE p/q} + \mathcal{L}_\text{TRE p/r} \right)$$

% \subsubsection{Different Instantiations}
% \begin{enumerate}
%     \item Shared optimizer, different classifier for each dataset
%     \item Shared model, different heads (fully multitask learner)
% \end{enumerate}

% \subsection{Simple Baselines}
% Something we should be keeping in mind is the fact that the original binary classification problem (logistic regression) leads to a Bayes optimal classifier. Therefore, we should make sure to thoroughly check simpler baselines (not necessarily involving consistency loss), as adding the consistency loss may yield a suboptimal solution.

% \subsubsection{One vs. All Binary Classifier}
% In this setting, we train a binary classifier to distinguish between $p$ vs. $\{q, r\}$ (a concatenated mixture of the two biased sources). We'll be testing whether the one vs. all classification problem (in the multi-class classification setting) gives us good results for density ratio estimation. \\

% Note that the ratio estimates we obtain are: $w(\bx) = \frac{p(y=1|x)}{p(y=0|x)}$, where $p(y=1|x)$ refers to samples from $x \sim p$ and $p(y=0|x)$ refers to samples from $x' \sim \{q,r\}$. We only need access to $w(\bx)$ for the purposes of fair generative modeling (e.g. up-weighting the target examples, and vice versa), rather than individual estimates $p/q, q/r$, etc.\\

% The classifier we learn in this setting is straightforwardly Bayes optimal.

% \subsubsection{Multi-class Classifier}
% In this setting, we train a softmax classifier to distinguish between $p, q, r$ separately. We'll be testing whether the one vs. one classification problem (in the multi-class classification setting) gives us good results for density ratio estimation. \\

% We'll be working with a 3-way classification problem, where we label the samples from $p$ as $y=1$, sample from $q$ as $y=2$, and samples from $r$ as $y=3$.\\

% Call the output logits for class $c$: $f(\bx)^T w_c$, where $f(\cdot)$ denotes a feature map $f: \mathcal{X} \rightarrow \mathbb{R}^d$ and $w$ denotes the weights of a k-way linear classifier $w: \mathbb{R}^d \rightarrow \mathbb{R}^{k}$. Note that the loss is now the straightforward softmax loss:
% $$\mathcal{L} = \frac{\exp(f(\bx)^T w_c)}{\sum_{c'} \exp(f(\bx)^T w_{c'})} = p(y=c|x) = \frac{p(x|y=c)}{\sum_{c'} p(x|y=c')}$$

% where we can see that this classifier is also Bayes optimal. The density ratio estimates that we want can be computed by taking $p(y=1|x)$ and dividing it by $(p(y=2|x) + p(y=3|x))$. Concretely, if exponentiating the output logits gave us a distribution such as \texttt{[0.6, 0.3, 0.1]}, then $p/(q+r) = .6/.4$.\\

% This baseline is very similar to the one vs. all binary classifier, except that we have separate class-conditional probabilities for the other biased datasets as well. \textbf{NOTE:} Refer to ESL 4.4, 14.2.4, and \texttt{https://arxiv.org/pdf/1805.09921.pdf} Appendix B for more details!

% \subsection{Consistency Loss}
% To make things a little more interesting, we can train a third classifier for the biased sources $\{q, r\}$ and regularize the loss to ensure that this third classifier obtains an output that is similar to the product of the ratios of the two other learned classifiers (from the previous section):
% $$\mathcal{L}_\text{Multi-Consistency-TRE} = \frac{1}{2}\left(\mathcal{L}_\text{TRE p/q} + \mathcal{L}_\text{TRE p/r} \right) + \lambda \left(\frac{p}{q} \times \frac{q}{r} - \frac{p}{r} \right)^2$$
% \kristy{fix the regularization term so that it's the output of the ratios, not the actual ratios}


\kristy{proofs in case notation is screwed up}
\begin{corollary}\label{lemma:cvf:unbiased}
Let $\Dc_p$ be $n$ i.i.d samples from density $p_X$, and $\Dc_q$ be $n$ i.i.d samples from density $q_X$. Let $\widehat{r}(\Dc_p,\Dc_q,\bx)$ be an unbiased estimator of $r(\bx) = \frac{p_X(\bx)}{q_X(\bx)}$ for any $p_X,q_X$, and let $f_\theta$ denote any invertible mapping. 
Then:
\[
\bx' \mapsto \widehat{r}(\{f_\theta(\bx_1),\cdots, f_\theta(\bx_n)\},\{f_\theta(\bx'_1),\cdots, f_\theta(\bx'_n)\},f_\theta(\bx'))
\]
is also an unbiased estimator of $\frac{p_X(\bx')}{q_X(\bx')}$ for any $p,q$.
\end{corollary}
\begin{proof}
Because it is unbiased we have
\[
E_{\Dc_p \sim p,\Dc_q \sim q } \left[ \widehat{r}(\Dc_p,\Dc_q,\bx) \right] = \frac{p(\bx)}{q(\bx)}
\]
Letting $p',q'$ be the densities of $f_\theta(X)$ and $f_\theta(Y)$ respectively we have
\[
E_{\Dc_p' \sim p',\Dc_q' \sim q' } \left[ \widehat{r}(\Dc_p',\Dc_q',f_\theta(\bx)) \right] = \frac{p'(f_\theta(\bx))}{q'(f_\theta(\bx))}
\]
and by definition of $p',q'$ this is equivalent to
\[
E_{\Dc_p \sim p,\Dc_q \sim q } \left[ \widehat{r}(f_\theta(\Dc_p),f_\theta(\Dc_q),f_\theta(\bx)) \right] = \frac{p'(f_\theta(\bx))}{q'(f_\theta(\bx))} = \frac{p(\bx)}{q(\bx)}
\]
where the last equality is due to Lemma 1.
\end{proof}

% \kristy{needs fixing, but can havea  corollary with this kind of flavor}
\paragraph{Consistency.}

\begin{corollary}\label{lemma:cvf:consistent}
Let $\Dc_p =\{\bx_1,\cdots, \bx_m\} \sim p$ be $m$ i.i.d samples from density $p$. Let $\Dc_q= \{\by_1,\cdots, \by_m\} \sim q$ be $m$ i.i.d samples from density $q$. Let $\widehat{r}(\Dc_p,\Dc_q,\bx)$ be a consistent estimator of $\frac{p(\bx)}{q(\bx)}$ for all $\bx$ and for any $p,q$. Let $f$ be any invertible mapping. 
Then
\[
\bx' \mapsto \widehat{r}(\{f_\theta(\bx_1),\cdots, f_\theta(\bx_m)\},\{f_\theta(\by_1),\cdots, f_\theta(\by_m)\},f_\theta(\bx'))
\]
is also a consistent estimator of $\frac{p(\bx')}{q(\bx')}$
\end{corollary}
\begin{proof}
Because it is consistent we have $\forall \bx, \forall \epsilon$
\[
\lim_{m \rightarrow \infty} P_{\Dc_p \sim p,\Dc_q \sim q } \left[
\left|\widehat{r}(\Dc_p,\Dc_q),\bx)-\frac{p(\bx)}{q(\bx) } \right| > \epsilon\right] = 0
\]
Let $p',q'$ be the densities of $f_\theta(X)$ and $f_\theta(Y)$ respectively. Because the estimator is assumed to be consistent for any $p,q$ we have
\[
\lim_{m \rightarrow \infty} P_{\Dc_p \sim p',\Dc_q \sim q' } \left[
\left|\widehat{r}(\Dc_p',\Dc_q',\bx)-\frac{p'(\bx)}{q'(\bx) } \right| > \epsilon\right] = 0
\]
and by definition of $p',q'$ this is equivalent to
\[
\lim_{m \rightarrow \infty} P_{\Dc_p \sim p,\Dc_q \sim q} \left[
\left|\widehat{r}(f_\theta(\Dc_p),f_\theta(\Dc_q),\bx)-\frac{p'(\bx)}{q'(\bx) } \right| > \epsilon\right] = 0
\]
Because the condition holds $\forall \bx$
\[
\lim_{m \rightarrow \infty} P_{\Dc_p \sim p,\Dc_q \sim q} \left[
\left|\widehat{r}(f_\theta(\Dc_p),f_\theta(\Dc_q),f_\theta(\bx))-\frac{p'(f_\theta(\bx))}{q'(f_\theta(\bx)) } \right| > \epsilon\right] = 0
\]
\[
\lim_{m \rightarrow \infty} P_{\Dc_p \sim p,\Dc_q \sim q} \left[
\left|\widehat{r}(f_\theta(\Dc_p),f_\theta(\Dc_q),f_\theta(\bx))-\frac{p(\bx)}{q(\bx) } \right| > \epsilon\right] = 0
\]
where the last equality is due to Lemma 1.
\end{proof}

% \begin{figure*}[!t]
%     \centering
%         \subfigure[Separate training (flow)]{\includegraphics[width=.33\textwidth]{figures/toy_gmm/toy_gmm_maf_z_encodings.png}}
%         \subfigure[Joint training ($\alpha=0.9$)]{\includegraphics[width=.33\textwidth]{figures/toy_gmm/toy_gmm_joint_a0.9_z_encodings.png}}
%         \subfigure[Discriminative training]{\includegraphics[width=.33\textwidth]{figures/toy_gmm/toy_gmm_disc_z_encodings.png}}
%     \caption{Visualizations of the learned encodings for various training strategies in Section~\ref{train_methods}. (a) Using a pre-trained flow as the feature map nicely partitions $p_X(\bx)$ and $q_X(\bx)$ in feature space. (b) Using a flow that is trained jointly with the classifier exhibits a similar, yet shifted, linear decision boundary between the encoded points. (c) The encodings from the discriminatively-trained model learns an arbitary warping of the two densities.}
%     \label{fig:gmm_encodings}
% \end{figure*}

% We provide some preliminary theoretical insights into why this is the case in Section~\ref{theory}.
% \kristy{would be nice to have a figure for these setups, or even just Algorithm 1}
% \kristy{unclear if still relevant}
% We note that our framework is quite general, in the sense that any pretrained flow that is trained on a mixture of $p(\bx)$ and $q(\bx)$ will suit our purposes. Concretely, we note that the density ratio estimate that we require may be obtained via importance reweighting, where the importance weights come from the distribution of our normalizing flow model:
% \begin{align*}
%     \mathbb{E}_{x \sim p(\bx)}\left[ g(\bx) \right] &= \mathbb{E}_{x \sim p_f(\bx)}\left[\frac{p(\bx)}{p_f(\bx)} g(\bx) \right]\\
%     &= \mathbb{E}_{x \sim p_f(\bx)}\left[\frac{p(\bx)}{\frac{1}{2} (p(\bx) + q(\bx))} g(\bx) \right] \\
%     &= \mathbb{E}_{x \sim p_f(\bx)}\left[\frac{r(\bx)}{\frac{1}{2} (r(\bx) + 1)} g(\bx) \right] \\
%     &= \mathbb{E}_{x \sim p_f(\bx)}\left[r'(\bx) g(\bx) \right]
% \end{align*}
% in a particular setting where our normalizing flow has been trained on an equal-sized mixture of $p(\bx)$ and $q(\bx)$. In the case that the mixing proportions are different, the importance weight $r'(\bx)$ can be recomputed accordingly. We refer the reader to Appendix \kristy{TODO} for more details (could potentially talk about this more).

% We note that an interesting consequence of our hybrid training approach is that our method gives the user the ability to \textit{sample} from the learned data density, whether it be from the mixture distribution that is learned by the normalizing flow $\left(\text{i.e. } p_f(\bx) = \frac{1}{2}p(\bx) + \frac{1}{2}q(\bx) \right)$ or from a specific target distribution of interest (e.g. $q(\bx)$) by reweighting the contribution of the sample.

% Structure:
% \begin{enumerate}
%     \item Position as general-purpose ``meta-algorithm" that takes in a density ratio estimation method and data
%     \item Train a flow on data and call density ratio estimation method
%     \item Should inherit good properties of the existing algorithm
% \end{enumerate}
% Some things we can show:
% \begin{enumerate}
    % \item Consequence of previous Proposition $(r(\bx) = r(\bz))$, we inherit these propertiees
    % \item Question: can we make this better if the algorithm depends on the distance between p and q?
% \end{enumerate}

% \subsection{Notation}
% For clarity of exposition, we introduce some additional notation that will be used throughout the paper. We let $Z_p$ denote the random variable resulting from the transformation of $X_p$ via $f_\theta$, such that $Z_p = f_\theta(X_p)$. $Z_q$ is defined analogously where $Z_q = f_\theta(X_q)$. We let $Z_p \sim p'$ and $Z_q \sim q'$. Additionally, we denote $Z = \frac{1}{2}Z_p + \frac{1}{2}Z_q$ with density $p_Z$. In particular, $p_Z$ represents the base distribution of the flow $f_\theta$.
% \se{not sure this is the right place for this..which flow is this talking about? not introduced yet}


% \kristy{this is where you should have the different random variables $Z, Z'$, talk about $z = f(x)$, etc.}
% \kristy{SAY SOMETHING ABOUT ZS HERE}
% \kristy{TODO: CLEAN UP NOTATION
% \begin{enumerate}
%     \item $p, q \rightarrow p',q'$
%     \item $z = f(x), z' = f(x'), f(x) \sim p_z, f(x') \sim p_{z'}$ 
%     \item $0.5p' + 0.5q' = \text{something else, NOT z as it's currently written}$ (give a different name)
% \end{enumerate}
% }
% Some items that we need:
% \begin{enumerate}
%     \item $Z_p = f_\theta(X_p) \sim p'$
%     \item $Z_q = f_\theta(X_q) \sim q'$
%     \item $Z = \frac{1}{2}Z_p + \frac{1}{2}Z_q \sim p_Z (?)$
% \end{enumerate}

% \kristy{am going to ignore the below comment bc we need to be careful about mentioning infinity ratios}
% \kk{maybe say something more concrete about how the density ratio explodes with the degree of mismatch between distributions? e.g. if you have two gaussians, how does the average density ratio between them scale with the mean/covariance? (this should be analytically expressable?)}

% \begin{figure*}[!t]
%     \centering
%         \subfigure[Ground truth data]{\includegraphics[width=.25\textwidth]{figures/toy_gmm/toy_gmm_data.png}}
%         \subfigure[Separate training (flow)]{\includegraphics[width=.25\textwidth]{figures/toy_gmm/toy_gmm_maf_z_encodings.png}}
%         \subfigure[Joint training ($\alpha=0.9$)]{\includegraphics[width=.24\textwidth]{figures/toy_gmm/toy_gmm_joint_a0.9_z_encodings.png}}
%         \subfigure[Discriminative training]{\includegraphics[width=.24\textwidth]{figures/toy_gmm/toy_gmm_disc_z_encodings.png}}
%     \caption{Visualizations of the learned encodings for various training strategies in Section~\ref{train_methods}. (a) Using a pre-trained flow as the feature map nicely partitions $p(\bx)$ and $q(\bx)$ in feature space. (b) Using a flow that is trained jointly with the classifier exhibits a similar, yet shifted, linear decision boundary between the encoded points. (c) The encodings from the discriminatively-trained model learns an arbitrary warping of the two densities. \kristy{clean up caption}}
%     \label{fig:gmm_encodings}
% \end{figure*}


% \begin{figure*}
%     \centering
%         \subfigure[True log ratios]{\includegraphics[width=.24\textwidth]{figures/toy_gmm/toy_gmm_true_log_r.png}}
%         \subfigure[Baseline classifier]{\includegraphics[width=.24\textwidth]{figures/toy_gmm/toy_gmm_hist_xclf.png}}
%         \subfigure[Discriminative training]{\includegraphics[width=.25\textwidth]{figures/toy_gmm/toy_gmm_hist_disc.png}}
%         \subfigure[Separate training (flow)]{\includegraphics[width=.25\textwidth]{figures/toy_gmm/toy_gmm_hist_flow.png}}
%     \caption{Motivating example on a synthetic 2-D Gaussian dataset. (a) Scatter plot of data and (b) true log ratios of the two Gaussians $p(\bx)$ and $q(\bx)$. (c) Training a probabilistic classifier on the data points directly fails to estimate the density ratios accurately. (d) After training a normalizing flow on both $p(\bx)$ and $q(\bx)$ and using it as an encoder, training a classifier on the encodings improves performance in density ratio estimation. \kristy{fix caption}}
%     \label{fig:gmm_encodings}
%     % \ys{A more extreme experiment shall look better. Maybe make the variance of two Gaussians even smaller?}
%     % \andy{axis labels for 2b and 2d would be helpful}
%     % \kristy{fix figure caption}
% \end{figure*}


==> sections/old_method.tex <==
\section{Featurized Density Ratio Estimation}
\label{method}

\subsection{Motivating Example and Intuition}
\kristy{RESTRUCTURING: current}
\begin{enumerate}
    \item here is a failure case
    \item our solution is a flow
    \item here is a lemma and pseudocode for how to use our method
    \item here are different training procedures
    \item here are the different feature spaces learned by the different training procedures
    \item here is a reason for why the flow is helping DRE
\end{enumerate}
\kristy{RESTRUCTURED}
\begin{enumerate}
    \item here is a failure case
    \item some intuition about why this is hard is because of the p,q example. so effectively we need to bring p,q closer together
    \item our solution is a flow
    \item here is a lemma and pseudocode for how to use our method
    \item here are different training procedures
    \item here are the different feature spaces learned by the different training procedures. visually, it looks like p,q won't ever be able to be super far apart, which we argue is good
\end{enumerate}
\subsection{Methodology}\label{method}
Despite the variety of existing techniques for density ratio estimation, they are of limited use
in settings where $p(\bx)$ and $q(\bx)$ are sufficiently different \citep{cortes2010learning,yamada2013relative,rhodes2020telescoping}
We highlight an illustrative failure case in Figure~\ref{fig:gmm_encodings} on a 2-dimensional toy dataset, where $p(\bx) \sim \mathcal{N}([0, 0]^T,I)$ and $q(\bx) \sim \mathcal{N}([3, 3]^T,I)$. As shown in Figure~\ref{fig:gmm_encodings}(e), the two random variables have regions of minimal overlap -- when training a binary classifier $c_\phi$ to distinguish the two sets of samples, the log-ratio estimates $\log \hat{r}_\phi(\bx)$ learned by the classifier are not accurate (Figure~\ref{fig:gmm_encodings}(a)). This empirical observation is in line with that of \citep{you2019towards,rhodes2020telescoping}, who also pointed to the mismatch between $p(\bx)$ and $q(\bx)$ as a major challenge in high-dimensional density ratio estimation. 

To address this problem, we consider training an invertible deep generative model $f_\theta$ on a \textit{mixture} of $p(\bx)$ and $q(\bx)$, such that $Z_p = f_\theta(X_p)$ and $Z_q = f_\theta(X_q)$ are mapped to a common feature space $\mathcal{Z}$. We note that $Z = \frac{1}{2}Z_p + \frac{1}{2}Z_q$ with density $p_Z$, where $p_Z$ represents the base distribution of the flow $f_\theta$.
The result of leveraging $f_\theta$ as invertible feature map can be visualized in Figure~\ref{fig:gmm_encodings}(f): we notice that the flow compresses all data points to lie in different regions of a unit Gaussian ball.
% However, when we train a normalizing flow $f_\theta$ on both datasets and use it to encode all examples into a shared feature space, we observe in Figure~\ref{fig:gmm_encodings}(c) that the flow squeezes the data points to lie in different regions of a unit Gaussian ball. 
By mapping regions of low density in $\mathcal{X}$ into regions of higher density in $\mathcal{Z}$, and training our probabilistic classifier $c_\phi$ on $f_\theta(\bx) \in \mathcal{Z}$ rather than $\bx \in \mathcal{X}$ directly, this contraction leads to more accurate density ratios as shown in Figure~\ref{fig:gmm_encodings}(b). We refer the reader to Appendix~\ref{addtl-results} for additional experimental details and results. 
% \kk{what's missing here is a characterization of a good feature space vs a bad one. How should one think about choosing a good latent space? I assume that not all invertible maps will lead to a good feature space, e.g identity map. Maybe it comes later but I'm constantly wondering this as I read this section} 

% \kristy{We can potentially cite \citep{rhodes2020telescoping} and other papers which talk about distance between p and q as a roadblock for getting good density ratio estimates. This will motivate our problem further.}

% \kristy{decide if we should put z-space representations here, or if we should move this example to Section 4.} The representations learned by our model and the baseline are shown in Figure~\ref{fig:gmm_encodings}.
% We consider training an invertible deep generative model $f_\theta$ on a \textit{mixture} of $p(\bx)$ and $q(\bx)$, such that $\bz = f_\theta(\bx)$ and $\bz' = f_\theta(\bx')$ are mapped to a common feature space $\mathcal{Z}$. 
To develop further intuition about this framework, our first observation is that as a direct consequence of the invertibility of $f_\theta$, the density ratios obtained in feature space are equivalent to those obtained in input space. We formalize this statement in Lemma~\ref{lemma:cvf} below.
\begin{lemma}\label{lemma:cvf}
Let $X_p \sim p$ be a random variable with density $p$, and $X_q \sim q$ be a random variable with density $q$. Let $f_\theta$ be any invertible mapping. Let $p',q'$ be the densities of $Z_p = f_\theta(X_p)$ and $Z_q = f_\theta(X_q)$ respectively.
Then for any $\bx$:
\[
\frac{p(\bx)}{q(\bx)} =  \frac{p'(f_\theta(\bx))}{q'(f_\theta(\bx))}
\]
\end{lemma}
\begin{proof}
We provide the proof in Appendix~\ref{lemma-proof}.
\end{proof}
This simple observation is quite powerful, as it lends us a general-purpose algorithm that may improve many existing ratio estimation techniques as a black-box wrapper. We provide the pseudocode for our training procedure in Algorithm~\ref{alg:fdre}. Given the two sets of samples, the ratio estimation method, and an invertible generative model, we first train the normalizing flow on a mixture of the two datasets (Lines 2-3). We then use the trained flow to encode the samples into a common feature space and plug them into the base density ratio estimator algorithm $\texttt{DRE}(\cdot)$ to obtain our featurized density ratio estimator $\hat{r} \circ f_\theta^*$, which is implicitly composed with the trained normalizing flow (Line 6).
% \se{i think this is not right, you need to return $\hat{r} \circ f_\theta$}
% and encode the samples into a common feature space (Line 5). Then, we call the density ratio estimation technique on the encoded data points and return the estimate after computing them in feature space as in Line 6.
% \kristy{some fixes:
% \begin{enumerate}
%     \item be more precise/add more detail in Algo 1, algo also returns function
%     \item Give density ratio estimator a name
%     \item dre takes in datasets, returns function
%     \item TODO: return a density ratio estimate at a point, or the function to be evaluated at that point?????
% \end{enumerate}
% }
% \ys{No line number for comments in the pseudo-code.}
% \kristy{TODO: straighten out the pseudocode with $r$, $\hat{r}$, etc...}
% \kristy{right now $\hat{r}(x)$ is an estimate of $r(x)$. in proofs, $\hat{r}$ takes in 2 datasets and a point. you could potentially define a separate function $\tilde{r} = \hat{r}(D_p, D_q): \mathcal{X} \rightarrow \mathbb{R}$ like currying}
\begin{algorithm}[H]
  \caption{Featurized Density Ratio Estimation}
  \label{alg:fdre}
  \textbf{Input:} Datasets $\mathcal{D}_p$ and $\mathcal{D}_q$, Density Ratio Estimation Algorithm $\texttt{DRE}$, Invertible Generative Model Family $\{f_\theta, \theta \in \Theta\}$\\
  \textbf{Output:} Featurized Density Ratio Estimator $\hat{r} \circ f_\theta^*$\\
  %e at $\bx$: $\tilde{r}(\bz)$ \kristy{maybe 2 objects} \\
\begin{algorithmic}[1]
\STATE $\triangleright$ Phase 1: Train invertible generative model
  \STATE Concatenate datasets $\mathcal{D} = \{\mathcal{D}_p, \mathcal{D}_q\}$
  \STATE \label{line:flow}Train $f_{\theta^*}$ on $\mathcal{D}$ via maximum likelihood
 \STATE \label{line:test} $\triangleright$ Phase 2: Obtain density ratio estimator
%  \kristy{old}
 %\STATE \label{line:encode}Encode data point $\bx$ using normalizing flow $\bz \leftarrow f_{\theta^*}(\bx)$
 %\STATE $\tilde{r}(\bz) \leftarrow \hat{r}(f_{\theta^*}(\mathcal{D}_p), f_{\theta^*}(\mathcal{D}_q), \bz)$ \\
 % \STATE {\bfseries return } $\tilde{r}(\bz)$
%  \kristy{new}
%  \STATE {\bfseries return } $\bx' \mapsto
%  \hat{r}(f_{\theta^*}(\mathcal{D}_p), f_{\theta^*}(\mathcal{D}_q), f_{\theta^*}(\bx'))$
 \STATE $\hat{r} = \texttt{DRE}(f_{\theta^*}(\Dc_p), f_{\theta^*}(\Dc_q))$
 \STATE {\bfseries return} $\hat{r} \circ f_\theta^*$
\end{algorithmic}
\end{algorithm}
% \andy{a little odd that r and f are inputs, and then you train f (but you don't train r?) Maybe the input should just be the datasets?}
% \kristy{The thing we're still not sure about: if p and q are closer, does DRE become easier? ( can we make this better if the algorithm depends on the distance between p and q?)}

\subsection{Training Procedure}
\label{train_methods}
\se{maybe cleaner to define a specialized variant for when DRE is the classifier based one? leave fully general before, and then say if you know what DRE does, you can try to adapt the flow to that. here we explore classification one (and leave KMM/KLIEP as future work)[perhaps not too hard to come up with a specialized joint training for them too, but no time for experiments of course]}
In the probabilistic classification setting, where we train a binary classifier $c_\phi$ to distinguish between $\Dc_p$ and $\Dc_q$, 

In practice, there are a variety of ways to implement the training procedure as outlined in Algorithm~\ref{alg:fdre}. The most general is \textbf{separate training}, which leverages a pre-trained flow $f_\theta$ as an encoder to map the inputs into a common feature space, prior to ratio estimation. This approach is capable of handling all parametric and non-parametric techniques which operate directly in input space.

Another procedure is \textbf{joint training}, where both the normalizing flow $f_\theta$ and the discriminative classifier $c_\phi$ are trained jointly via the following objective:
\begin{equation} \label{joint_obj}
    \mathcal{L}_{\textrm{joint}}(\theta,\phi) = \alpha \mathcal{L}_{\textrm{sup}}(\theta,\phi) + (1-\alpha) \mathcal{L}_{\textrm{flow}}(\theta)
\end{equation}
where $\mathcal{L}_{\textrm{sup}}$ denotes the standard binary cross entropy (logistic) loss, $\mathcal{L}_{\textrm{flow}}$ denotes the maximum likelihood objective for the flow $f_\theta$, and $\alpha \in [0,1]$ is a tunable hyperparameter which balances the importance of the two terms in the loss function. This training approach is quite common in learning deep hybrid models \citep{kuleshov2017deep,nalisnick2019hybrid}. 
% \ys{This seems to be an application of tre, rather than a way to train the flow model or the classifier?}\kk{agree, seems misplaced}
% We refer the reader to Appendix~\ref{dre_details} for more details.

Finally, we explore \textbf{discriminative training}, where we modify the classifier $c_\phi$'s architecture to incorporate that of the flow $f_\theta$
% compose the classifier $c_\phi$ with the flow architecture $f_\theta$ 
to build an ``invertible" classifier $c_{\phi,\theta}: \mathcal{X} \rightarrow [0,1]$ that is trained solely via the logistic loss $\mathcal{L}_\textrm{sup}(\theta,\phi)$. 
% \kk{when you say "compose", it sounds like you are doing $c_{\theta, \phi} = c_{\phi} \circ f_{\theta}(x)$ where $f_{\theta}$ is a flow and $c_{\phi}$ is any (potentially non-invertible) function. I assume what you meant is that the entire classifier has the flow architecture and is invertiblem, so maybe clarify the wording?} 

\subsection{Characterization of the Learned Feature Space}
% \kristy{overall structure:}
% \begin{enumerate}
%     \item from Lemma~\ref{lemma:cvf}, we expect any invertible mapping to work
%     \item However, this is not the case (discriminative training fails miserably)
%     \item Maximum likelihood training of flow seems crucial for good performance
%     \item here are some plots you can look at (Figure~\ref{fig:gmm_encodings})
%     \item can we provide some justification for joint training?
%     \item goal: characterization of a "good" feature space vs a "bad one"
% \end{enumerate}
% \kristy{some things that you need to clarify in this section:}
% \begin{enumerate}
%     \item what makes a "good" feature space?
%     \item why is the discriminative baseline so bad?
%     \item why do we need maximum likelihood training?
%     \item you may consider moving this section up before "Training Procedure"
% \end{enumerate}
To gain some preliminary insight into the desirable characteristics of the learned feature space, we qualitatively analyze the encodings of the various training strategies in Figure~\ref{fig:gmm_encodings}. From Lemma~\ref{lemma:cvf}, we expect \textit{any} feature space induced by an invertible map to work well for density ratio estimation -- that is, we do not expect to see significant performance degradation across the three (separate, joint, discriminative) training procedures. We note that for both a pretrained (Figure~\ref{fig:gmm_encodings}(f)) and jointly trained (Figure~\ref{fig:gmm_encodings}(g)) normalizing flow, the data points are mapped to lie closer together in different regions of the unit Gaussian ball. However, for the discriminatively trained classifier that is equipped with an invertible ``encoder" module (Figure~\ref{fig:gmm_encodings}(h)), the data points are mapped to arbitrary regions in feature space and more closely resemble the shape of the original inputs (Figure~\ref{fig:gmm_encodings}(e)).
This observation, combined with the low quality density ratio estimates in Figure~\ref{fig:gmm_encodings}(d) relative to the other training methods (Figure~\ref{fig:gmm_encodings}(b-c)), suggests that maximum likelihood training of the normalizing flow $f_\theta$ is crucial for obtaining accurate density ratios in feature space. 

\se{should this stuff go towards the beginning of 3.2?}

\kristy{here is a thought dump.} We provide some intuition on why transforming the inputs using the normalizing flow helps improve density ratio estimation. Suppose we have two distributions, $p \sim \mathcal{N}(m,1)$ and $q \sim \mathcal{N}(-m,1)$, and we want to train a logistic regression model to tell apart these two. Suppose we have a finite number of samples for both distributions. When training the logistic regression model, we use maximum likelihood; that is, we maximize the objective:
$$\max_{w_0, w_1}\mathbb{E}_p[\sigma(w_1*x + w_0)] - \mathbb{E}_p[\sigma(w_1*x + w_0)]$$
Suppose that $m$ is large -- there is a large separation between $p$ and $q$. In this case, most samples from $x_p \sim p$ will be positive, and most samples from $x_q \sim q$ will be negative. In this scenario, to maximize the objective, the model will be incentivized to push $w_1 \rightarrow \infty$, which would lead to very inaccurate density ratio estimates. (In this 1-D Gaussian case, the density ratios would be $p(x)/q(x) = \exp \left[\frac{(x-m)^2 - (x+m)^2}{2} \right] = \exp[-2xm]$.) \kristy{link $w_1$ back to density ratio and show how it being $\infty$ is bad}

In fact, the probability that all samples from $x_p \sim p$ will be positive, and all samples from $x_q \sim q$ will be negative (if we have $n$ samples) is 
$$P(X_p > 0) \geq 1 - \exp(-m^2/2)$$
for a single sample, which means that for the entire training set of size $n$, the probability becomes
$$\prod_{i=1}^{n}P(X_p > 0) \geq (1 - \exp(-m^2/2))^n$$
(The same argument holds for seeing a sample that is negative for $q$). Therefore, the probability that we observe a sample from $p$ (and vice versa from $q$) that is less than or equal to 0 is: 
$$1-P(X_i>0 \forall i) \leq 1 - (1 - \exp(-m^2/2))^n$$ 
which means that we observe $X_i \leq 0$ w.p. $\leq \delta$ for $n < \frac{\log(1-\delta)}{\log(1-\exp(-m^2/2))}$. 

Therefore the greater the gap between $p$ and $q$ (so the larger the $m$), the less likely it is that we will be seeing points closer to the decision boundary (which will be located at $2m$), and therefore we are very unlikely to learn accurate density ratio estimates. (We'll need an extremely large training set size to learn accurate density ratios) From a visual inspection of Figure~\ref{fig:gmm_encodings}, we see that when we use the flow $f_\theta$ to map the datasets $\Dc_p$ and $\Dc_q$ into the shared latent space, the gap between the two densities shrinks considerably, making it much less likely for this kind of pathological behavior to happen. We save an in-depth theoretical analysis of this phenomenon for future work. \kristy{We refer the reader to Appendix~\ref{intuition} for additional details.}
% We investigate empirically whether endowing the classifier with the functional form of the invertible transformation suffices for learning accurate density ratios downstream -- perhaps not surprisingly, \kk{I think this is actually a bit surprising because there has been no discussion of what a good "feature space" is. If any feature space induced by an invertible encoder is good, then you can think of the early layers of your invertible classifier as the "encoder", so it should work well. Seems like what's important is how you choose the latent space, therefore the maximum likelihood objective matters} we find that generative training of the flow $f_\theta$ is necessary for good performance. 
% We provide such additional results in Appendix~\ref{addtl-results}.

% To gain some insight into the learned feature space of the normalizing flows, we visualize the encodings of various training strategies in Figure~\ref{fig:gmm_encodings}. We note that for both a pretrained (Figure~\ref{fig:gmm_encodings}(a)) and jointly trained (Figure~\ref{fig:gmm_encodings}(b)) normalizing flow, the data points are mapped to lie closer together in different regions of the uniform Gaussian ball. However, for the discriminatively trained classifier (with a flow component in the architecture), the data points are mapped to arbitrary regions in feature space that do not resemble the flow's Gaussian prior. This observation, combined with the low quiality density ratio estimates in Figure~\ref{fig:toy_gmm_encodings2}(d), suggests that the generative training of the normalizing flow is important for obtaining accurate density ratios in feature space. 

% \kk{not sure i understand what's the motivation for joint training? if the loss is disentangled into separate losses for theta and phi, why optimize them together? Especially if you claim that having the a good feature space is a critical for good density ratio estimation, then it seems like the initial iterations of training with the joint objective will be a waste of time since the feature map has not been fully learned yet and estimating density ratio in a bad feature space will not work well}

% \kk{what's missing here is a characterization of a good feature space vs a bad one. How should one think about choosing a good latent space? I assume that not all invertible maps will lead to a good feature space, e.g identity map. Maybe it comes later but I'm constantly wondering this as I read this section} 
